Efficient Quantization Strategies for Latent Diffusion Models

Latent Diffusion Models (LDMs) capture the dynamic evolution of latent variables over time, blending patterns and multimodality in a generative system. Despite the proficiency of LDM in various applications, such as text-to-image generation, facilitated by robust text encoders and a variational autoencoder, the critical need to deploy large generative models on edge devices compels a search for more compact yet effective alternatives. Post Training Quantization (PTQ), a method to compress the operational size of deep learning models, encounters challenges when applied to LDM due to temporal and structural complexities. This study proposes a quantization strategy that efficiently quantize LDMs, leveraging Signal-to-Quantization-Noise Ratio (SQNR) as a pivotal metric for evaluation. By treating the quantization discrepancy as relative noise and identifying sensitive part(s) of a model, we propose an efficient quantization approach encompassing both global and local strategies. The global quantization process mitigates relative quantization noise by initiating higher-precision quantization on sensitive blocks, while local treatments address specific challenges in quantization-sensitive and time-sensitive modules. The outcomes of our experiments reveal that the implementation of both global and local treatments yields a highly efficient and effective Post Training Quantization (PTQ) of LDMs.

==> sec/2_relatedwork.tex <==
\section{Related Work}
\label{sec:related}

\subsection{Efficiency of LDMs}
\label{subsec:efficiency}
DMs \cite{sohl2015deep,ho2020denoising} iteratively eliminate random noise in the pixel space to generate clean images. LDMs \cite{rombach2022high} enhance training efficiency by adapting denoising progress in the latent space. While efforts propose faster solvers to reduce inference requirements \cite{nichol2021improved,song2020denoising,lu2022dpm}, the model size and image generation time remain bottlenecks for light deployment. To address this, a combination of pruning, distillation, quantization, and hardware optimization is applied for LDM deployment on edge devices \cite{li2023snapfusion,choi2023squeezing}. \cite{fang2023structural} identifies weighted diffusion steps and structurally prunes the pretrained model, achieving a smaller size. \cite{li2023snapfusion} employs unstructural pruning and other techniques to enhance inference efficiency. Similarly, \cite{li2023efficient,bolya2023token,moon2023early} reduce redundancies in the structure of UNet or inference algorithm. \cite{salimans2022progressive,meng2023distillation} progressively distill LDMs to learn a lighter model generating comparable images in $\leq{2}$ inference steps. While these methods require additional training and access to original data, \textbf{quantization} reduces size and enhances efficiency with minimal retraining. This work focuses on refining the quantization of LDMs.

\subsection{Quantization of LDMs}
\label{subsec:quantization}
Quantizing LDM entails precision reduction in numerical representations to boost model efficiency and minimize operational size, with PTQ further refining the model post-initial training using calibration data. While quantization on Large Language Models (LLMs) exhibits promising compression results \cite{xiao2023smoothquant,bai2022towards}, adapting it to LDMs faces unique challenges due to their iterative and dynamic denoising steps, xacerbating to quantize activations containing dynamic outliers through simple linear quantization. Prior works \cite{li2023q, he2023ptqd, wang2023towards} address these challenges by selecting uniformly distributed calibration data across inference timesteps, dealing dynamic activation ranges with optimized quantization methods. In this paper, we offer a thorough analysis to present an efficient and effective quantization strategy that enhances performance, even with simple linear quantization.
